On the Inability of Markov Models to Capture Criticality in Human Mobility

We examine the non-Markovian nature of human mobility by exposing the inability of Markov models to capture criticality in human mobility. In particular, the assumed Markovian nature of mobility was used to establish a theoretical upper bound on the predictability of human mobility (expressed as a minimum error probability limit), based on temporally correlated entropy. Since its inception, this bound has been widely used and empirically validated using Markov chains. We show that recurrent-neural architectures can achieve significantly higher predictability, surpassing this widely used upper bound. In order to explain this anomaly, we shed light on several underlying assumptions in previous research works that has resulted in this bias. By evaluating the mobility predictability on real-world datasets, we show that human mobility exhibits scale-invariant long-range correlations, bearing similarity to a power-law decay. This is in contrast to the initial assumption that human mobility follows an exponential decay. This assumption of exponential decay coupled with Lempel-Ziv compression in computing Fano's inequality has led to an inaccurate estimation of the predictability upper bound. We show that this approach inflates the entropy, consequently lowering the upper bound on human mobility predictability. We finally highlight that this approach tends to overlook long-range correlations in human mobility. This explains why recurrent-neural architectures that are designed to handle long-range structural correlations surpass the previously computed upper bound on mobility predictability.

==> acknowledgments.tex <==
\section*{Acknowledgments}

This research work was partially supported by the Swiss National Science Foundation grant 157160.
This research was also supported by the ADAPT Research Centre, funded under the SFI Research Centres Programme (Grant 13/ RC/2106) and is co-funded under the European Regional Development Funds. 
The research was also supported by an IBM Shared University Research Award.

==> authors.tex <==
\section*{Author contributions}
V.K. and A.M. designed the research. 
V.K. performed the experiments. 
V.K., A.M. and B.G. wrote the manuscript. 
B.G. and J.D.K critically read the manuscript.

==> criticality_mobdata.tex <==
\section{Criticality in Mobility Data}

In this section, we discuss the relationship between mutual information and criticality.
We look at a result stated in Lin et al.~\cite{lin2016critical}, work "mutual information between two symbols, as a function of the number of symbols between the two, decays exponentially in any probabilistic regular grammar, but decays like a power law for a context-free grammar".
It is important to note here that, although for very short distances, power decay and exponential decay look more or less similar.
Thus, if predictive models were originally studied only for short sequences in the past, it seems to make sense that this is a mistake that anyone could have made more easily back then.
This refers to studying mobility behaviors for short durations, typically lasting 2-3 months using CDR datasets.

The number of bits of information provided by a symbol about another drops as a power-law with distance in sequences.
This distance is defined as the number of symbols between the two symbols of interest.
However, this power law is not the same power law occurring in natural languages~\cite{chomsky1959certain}.
Zipf's law implies power law behavior in one-point statistics, however mobility behaviors can be better described by two-point statistics.
As it involves implicit behavioral dynamics while traveling from a given location to other locations with a specific intent.
In the former case the power law is in the frequency of elements; however in the latter case the power law is in the separation between the elements.

Markov models of natural languages, have been shown fundamentally unsuitable for modeling human language~\cite{chomsky1959certain}.
However, linguistic models do not produce observable that can be used to quantitatively falsify Markovian models.
But these arguments rely on domain specific knowledge (for example understanding language grammar).
However, mutual information is trivial to observe, which requires no specific knowledge about the data, which indicates that natural languages will be poorly approximated by Markov models.


Mutual information decay offers some explanation as to why RNN-LSTMs are successful to replicate criticality.
It has also been shown that Markov Processes exhibit exponential decay in mutual information with scale~\cite{lin2016critical}.
Lin et al.~\cite{lin2016critical} also define another metric {\it{Rational mutual information}}, which bounds the mutual information and converges to it in the near independence limit.


In our case, the mutual information between two random variables is realization of a discrete stochastic process, with some separation $\tau$ in time.
We consider a time series of pairs $(x_1,y_1), (x_2,y_2),...,(x_N,y_N)$.
The points $x_n$ are selected independently from some $P(x)$ while the $y_n$ are noisy examples of a function $f(x)$, such that $y_n = f(f_{x_n} + \eta_n)$ with the $\eta_n$ chosen, for example from a Gaussian distribution. 
Now, we need to assume that the function $f(x)$ can be written as a sum of $K$ basis functions $\phi_1(x), \phi_2(x),...,\phi_K(x)$ with some unknown coefficients $c$.
The joint probability distribution of ${x_n,y_n}$ can be estimated.
Here, $x_n$ be the timestamp and $y_n$ the discretized location coordinate.


{\bf{Mutual information and Markov Process.}} We refer to Theorem 1 from Lin et al.~\cite{lin2016critical}, which states If $M$ is irreducible and aperiodic then the asymptotic behavior of $I$ is exponential decay towards zero.
However if $M$ is reducible or periodic, $I$ can decay to a constant.
Therefore No Markov process whatsoever can produce a power-law decay.


This paper~\cite{lin2016critical} shows that an irreducible and aperiodic Markov process with non-degenerate eigenvalues cannot produce critical behavior, as the $I$ decays exponentially.
This phenomenon has been proved for a number of practical cases for the the degenerate case, the reducible case, the periodic case, detailed balance case, hidden Markov models.
The fundamental problem of Markov model is lack of memory, which is superficially overcome by redefining the state space to include symbols from the past.
This gives  false impression of success when the sequence under consideration lasts for a short duration but fails when larger duration datasets are considered. 
It also results in scale-invariance and state-space explosion.
Extending the above theorem to HMMs, no probabilistic regular grammar exhibits criticality.


Considering Bayesian nets, the mutual information tends to be dominated by the shortest paths via a common ancestor, whose length is $\delta$.
So far we have, HMM exhibit exponential decay, whereas probabilistic context free grammers can exhibit power law decays.
Human mobility clearly exits context-free nature and can be identified and codified. 
Mmeasuring the $I$ as a function of separation between symbols is a computationally efficient way of extracting much more meaningful information about performance of a model than simply evaluating the loss function.
Lin et al.~\cite{lin2016critical} also shows that, higher order Markov models needs more parameters than LSTM-RNN and it captures less than one fifth of the mutual information captured by the recurrent-network architectures.

==> entropy_predictability.tex <==
\section{Accuracy Charts}

The current approaches related to estimating the limits of predictability of human mobility conclude that the bounds of error probability are correlated with: 
\begin{enumerate}
	\item Movement entropy 
	\item Number of unique location traversed by a user 
	\item Temporal resolution of the user trajectory data
	\item Spatial resolution of the user trajectory data
\end{enumerate}

Therefore, when a point is reached where further substrings are not unique anymore, the string matching algorithm sets the length of the substring to zero.

The movement entropy denoted as true entropy $S^{real}$ is estimated depending on the order in which the locations are visited by a user along with the dwelling time at each location.
Such an approach captures the complete spatiotemporal order present in a user's mobility pattern.\\

If $U_i = {X_1, X_2...X_L}$, where $U_i$ denotes the sequence of locations visited by user $i$ at consecutive hourly intervals, the entropy is given by

\begin{equation}
	-\sum_{{T_{i}}^{'}\subset T_i}P({T_{i}}^{'}).log_{2}[P({T_{i}}^{'})]
\end{equation}

,where $P({T_i}^{'})$ is the probability of finding a particular time ordered subsequence, ${T_{i}}^{'}$ in the user trajectory $T_{i}$.\\

This entropy is estimated using Lempel-ziv compression~\cite{lu2013approaching}, which converges to true entropy only when the number of items (locations in our case) approach infinity.
The CDR datasets used in the works~\cite{Song2010LimitsOP, lu2013approaching} have inherent gaps due the short bursts of calls which would mask the user's true entropy.
Thus adding noise to the estimation, directly affecting the true entropy.\\

The predictability upper bound (bottomline for error bound) is estimated using Fano's inequality~\cite{ho2008conditional, prelov2008mutual}.
In a nutshell, Fano's inequality relates the conditional entropy of a random variable $X$ relative to the correlated variable $Y$ to the probability of incorrectly estimating $X$ from $Y$.\\

Some notations to explain the main problem:
\begin{enumerate}
	\item Shanon information content of an outcome of a random variable: $log_{2}\frac{1}{p(x)}$
	\item Entropy: average uncertainty in random variable X: $H(X) = E_{p}.[log_{2}\frac{1}{p(x)}]$
	\item Conditional entropy between two variable $H(Y|X) = E_{p(x,y)}.[log_{2}\frac{1}{p(y|x)}]$
	\item Relative entropy: $D(p||q) = E_{p}[log_{2}\frac{p(x)}{p(y)} ]$
	\item Mutual Information between two random variables $X,Y: I(X,Y) = D(p(x,y)||p(x)p(y))$
\end{enumerate}

Now, consider a Markov process such that $X,Y,Z$ form a Markov chain in the order $X \rightarrow Y \rightarrow Z$ iff $p(x,y,z)=p(x)p(y|x)p(z|y)$. Resulting scenarios:

\begin{enumerate}
	\item  $X \rightarrow Y \rightarrow Z$ iff $X$ and $Z$ are conditionally independent given Y
	\item  $X \rightarrow Y \rightarrow Z$ and $Z \rightarrow Y \rightarrow X$. Thus we can say  $X \leftrightarrow Y \leftrightarrow Z$
	\item  if $Z = f(Y)$, then $X \rightarrow Y \rightarrow Z$ 
\end{enumerate}


In case of human mobility trajectories, we consider $X \rightarrow Y \rightarrow Z$ implying $I(X;Y) \geq I(X;Z)$, leading to a statistical inference as $X \rightarrow Y \rightarrow \hat{X}$ such that $\hat{X}=g(y)$, where $\hat{X}$ is an estimator of $X$, $\hat{X} = g(Y)$ therefore $I(X,Y) \geq I(X,\hat{X})$.\\

Assuming the random variable $X$ and its estimator $\hat{X}$ take up to $k$ different values.
Considering the case when $X$ and $\hat{X}$ are not equal (incorrect prediction of X).
Probability of error is thus: $P_{e} = P_r(\hat{X} \neq X)$.
Indicator function for error $E$ which is 0 when $X = \hat{X}$ and 1 otherwise.
Thus, $P_e = P(E=1)$. 
Fano's inequality is thus $H(E) + plog(k) \geq H(X|Y)$, the weaker result can be formulated as $p \geq \frac{H(X|Y)-1}{log(k)}$, the entropy of the binary event $E$ is atmost 1.
It is thus clear that the probability of incorrectly predicting the value of $X$ based on the information from $Y$ is constrained by the remaining uncertainty $H(X|Y)$ about $X$ when $Y$ is known.

The two possible cases here are when $X$ and $Y$ are independent in which case $H(X|Y) = H(X)$ and the probability of error depends on the certainty of $X$.
Under a uniform distribution of $k$, $p \geq 1 - \frac{1}{log(k)}$.
Therefore as k grows the predictability reduces ad the probability of making errors increase.
Conversely, when $p=0$, the conditional entropy is necessarily 0, and $X$ is perfectly known given $Y$.


In practice, this error probability (predictability) is computed by segmenting the entire trajectory in sub-strings, where the length of the shortest substring beginning at position $i$, does not appear previously~\cite{lu2013approaching, Song2010LimitsOP, smith2014refined, ikanovic2017alternative} .
Therefore, when a point is reached where further substrings are not unique anymore, the string matching algorithm will estimate the length of the substring to be 0.
The total predictability, $\pi^{max}$ is than estimated by averaging the individual error probabilities. 

The important point to note here, is that when the trajectory is split in to short substrings, the entropy associated with the individual strings increases due to removal to long distance dependencies, therefore consequently increase $p$ and consequently reducing $\pi^{max}$.
This occurs as Fano's inequality rooted in information theory in its true form was meant to be applied to a true data sequence whose true distribution is known and not to sampled sequences such as human mobility trajectories. 
When applied to short subsequences, would naturally increase the true entropy of a user's trajectory.
This value applied in its current form acts a limit on Markov models. 


We show that, instead of splitting the trajectory based on the uniqueness criterion, the subsequences having identical long distance correlation entropy should be clustered together to compute the error probability. 
Such a scheme retains the true entropy in a sequence which is lower than the currently used technique, which results in bounds higher than the once computed by Fano's inequality.
The resulting higher predictability bounds explain the superior performance of recurrent neural architectures as compared to Markov chains bounded by Fano's inequality in its current form. 




We show that, instead of splitting the trajectory based on the uniqueness criterion, the subsequences having identical long distance correlation entropy should be clustered together to compute the error probability. 
Such a scheme retains the true entropy in a sequence which is lower than the currently used technique, which results in bounds higher than the once computed by Fano's inequality.
The resulting higher predictability bounds explain the superior performance of recurrent neural architectures as compared to Markov chains bounded by Fano's inequality in its current form. 






%They achieve a tighter bound on predictability by removing impractical transitions from the potential transition set consequently increasing the movement entropy.  
%They also point out that while estimating the entropy, the generating function behind the stochastic process is unknown and therefore the theoretical estimation of entropy is impractical and necessitate the derivation empirically. 
%On the contrary, They compute the entropy by extrapolating from the missing data and show that is directly dependent on the number of unique locations visited by a user.


%The presence of heavy tails in human dynamics was shown by Barabasi~\cite{barabasi2005origin} as the subsequent locations are selected by a user based on some perceived priority.
%In such a case, most tasks are rapidly executed, whereas few location visits have long waiting times.
%It is shown that such processes can be categorized as non-Poisson. 
%Kingman et al.~\cite{kingman1963exponential} shows that n-step transition probabilities of a discrete-time Markov chain achieves exponential convergence to its ergodic limit. 

==> info.tex <==
\section*{Additional Information}
{\bfseries{Competing financial interests:}} The authors declare no competing financial interests.

==> markov_processes.tex <==
\section{Markov Processes \& Exponential Decay}


Stochastic processes are often characterized in terms of the transition probabilities where the probability for transitioning to the next state is an exponentially distributed random variable. 
For example $a \rightarrow b$ at probability $\alpha$ and $b \rightarrow a$ at rate $\beta$, i.e. the process transitions from state $a$ to $b$ with an exponential probability distribution with a mean of $\frac{1}{\alpha}$.
The stationary distribution for this trivial process is $\pi(a) = \frac{\beta}{\alpha+\beta}$ and $\pi(b) = \frac{\alpha}{\alpha+\beta}$.


However, we consider a scenario in which the probability distributions are not exponentially distributed.
Let, $\tau_{ab}$ be the transition probability from state $a$ to state $b$.
Let the distributions be given by $\tau_{ab} ~ f(t)$ and $\tau_{ba} ~ g(t)$ so that $p(\tau_{ab} \in A) = \int_{A}f(t)d(t)$.
We examine the stationary distribution of such a process, the transient dynamics of the transition probabilities and the limiting or stationary distributions~\cite{johnson2013bayesian}.







The exponential distribution is the only continuous distribution with the memory-less property~\cite{cflsp}. 
In order for a process to have a non-exponential probability and satisfy the Markov property, the precise transition probability given the current state must be known.
If a process has two or more states and transitions from each state with some non-exponential probability, then knowledge of the current state will not be enough to estimate the future distribution.
Furthermore if the transition probabilities are neither independent and identical (i.i.d) nor exponential, then in general the existence of either stationary distribution or a limiting distribution cannot assumed with certainty.


The number of hidden states must be set a priori so that model complexity is not inferred from data in a Bayesian way.
The Markovian disadvantage is even compounded in the nonparametric setting, since non-Markovian behavior in data can lead to the creation of unnecessary extra states and unrealistically rapid switching dynamics.
One serious limitation of the standard HDP-HMM (hidden Markov models) is that it inadequately models the temporal persistence of states. 
This problem arises in classical finite HMMs as well, where semi-Markovian models are often proposed as solutions.  
However, the problem is exacerbated in the nonparametric setting, where the Bayesian bias towards simpler models is insufficient to prevent the HDP-HMM from learning models with un-realistically rapid dynamics~\cite{fox2008hdp}.

==> predictive_info.tex <==
\section{Predictive Information}

Predictive Information, measures and quantifies how much of the past observations (can) tell us about the future (relies on information theory).
In case of sequential data, predictive information diverges when the observed series allows to learn a more more precise model of the data dynamics.
The structure of this divergence can measure a model's complexity~\cite{bialek1999predictive}.

Different kinds of predictions are different slices through the conditional probability distribution..
Greater concentration of this conditional distribution implies smaller entropy than the prior distribution.
This reduction in entropy is Shanon's definition of the information that the past provides about the future~\cite{shannon1951prediction}.
The average of this predictive information is:

\begin{equation}
\begin{aligned}
\label{eq:eq9}
I_{pred}(T) = log_{2}[\frac{P(X_{future}, X_{past})}{P(X_{future}P(X_{past}))}] \\
& = -(log_2.P(X_{future}))-(log_2.P(X_{past}))-[-(log_2.P(X_{future},X_{past}))]
\end{aligned}
\end{equation}

Furthermore, in a time series if there is invariance under time translations, the entropy of the past data depends only on the duration of the observations.
As a result, Equation~\ref{eq:eq9} is:

\begin{equation}
	\label{eq:eq10}
	I_{pred}(T) = 2S(t)-S(2T)
\end{equation}

{\bfseries{The entropy of a time series is therefore in direct proportion to the observed duration.}}
Therefore, using a dataset of duration lasting only 3 months will result in a false sense of entropy. which is further degraded by splitting the trajectories into sub-strings. 
In other words, entropy is the minimum number of bits required to describe the past data.
Predictability of a time series is therefore associated with deviation of the entropy from extensivity.
In Equation~\ref{eq:eq10} the extensive components cancel each other out and therefore the predictive information must be sub-extensive.
Therefore:

\begin{equation}
	\label{eq:eq11}
	\lim_{T \rightarrow \infty} I_{pred}(T)/T = 0
\end{equation}

and  

\begin{equation}
	\label{eq:eq12}
	\lim_{T \rightarrow \infty}{\frac{I_{pred}}{S(T)}} \rightarrow 0
\end{equation}

As a result most of what is observed is irrelevant to the problem of predicting the future.
Now, predictive information can behave in three ways, 

\begin{itemize}
	\item One when $T$ is large, $\lim_{T \rightarrow \infty} I_{pred}(T) = K$, where $K$ is some constant
	\item Predictive information is small as dynamics are too regular, this occurs when there is a high periodicity (movement regularity) involved
	\item In practice, however, there are critical points where the correlation times becomes infinite, therefore the predictions will be influenced by events from distant past (long-distance dependencies) andtherefore the predictive information can grow without bounds as $T \rightarrow \infty$  
\end{itemize}

For practical systems, the divergence is logarithmic, i.e. $I_{pred}(t \rightarrow \infty) ~ \mu.ln(T)$.
Consider a series $x(t)$ at a series of discrete times ${t_n}$, and that each time point we find the value of $x_n$.
The joint distribution of $N$ data points can be given by:

\begin{equation}
	\label{eq:eq13}
	P(x_1,x_2,...,x_N) = P(x_1)P(x_2|x_1)P(x_3|x_2,x_1)...
\end{equation}


For Markov processes, the observations at $t_n$ depends only on events at previous time step $t_{n-1}$ or on previous $n$ time steps for $n$-order Markov chain.
The maximum possible predictive information is the entropy of the distribution of states at one time step, which is bounded by the logarithm of the number of accessible states.
In order to approach this bound, the system must maintain memory for a very long time, as the predictive information is reduced by the entropy of the transition probabilities.
Therefore, systems with more states and longer memories have larger $I_{pred}$.


As we observe more of the time series, we expect to provide a more sophisticated description of the underlying function, increasing the number of parameters in the model with time.
Predictive information therefore is proportional to the number of parameters, and grow rapidly with $N$ in a nonparametric setting.
Therefore, when we examine mobility trajectories, on the scale of individual coordinate points, we learn about the rules of combining the points into stay points and paths between them.
But, if we look at hundreds of stay points and paths we also learn about the rules for combining these points in to semantic patterns and transportation modes.
Similarly, when we look at semantic patterns and transportation modes, we can learn about periodicities in visitations and circadian rhythms associated to mobility behaviors.
Therefore longer traces teach us an increasing number of different things, rather than giving us more precise knowledge about a fixed number of rules or parameters.
Statistical analysis, suggests that entropy associated to long trajectories have a large sub-extensive component and that this component and hence the predictive information - is best fit by a power law, so that $I_pred \propto N^{1/2}$ for $N$ coordinate points.


The average amount of information, we have about the current state of a time-series is independent of how long we have been watching.
However, if the signal has diverging predictive information then the space required to write down the model description grows as we observe the world for longer periods of time.
Therefore, if we observe for a very long time then the amount that we know about the future will exceed, by a large factor, the amount that we know about the present.
$I_{pred}$ therefore distinguishes processes that can be described by a finite number of parameters from those that cannot, and counts the number of parameters (dimensions) that are relevant.
For models with a finite number of parameters, the stochastic complexity is proportional to the number of parameters and logarithmically dependent on the number of data points $N$~\cite{shannon1951prediction,hilberg1990bekannte}.

==> related_work.tex <==
\section{Related work}


